On the Utility of Accounting for Human Beliefs about AI Intention in Human-AI Collaboration

To enable effective human-AI collaboration, merely optimizing AI performance without considering human factors is insufficient. Recent research has shown that designing AI agents that take human behavior into account leads to improved performance in human-AI collaboration. However, a limitation of most existing approaches is their assumption that human behavior remains static, regardless of the AI agent's actions. In reality, humans may adjust their actions based on their beliefs about the AI's intentions, specifically, the subtasks they perceive the AI to be attempting to complete based on its behavior. In this paper, we address this limitation by enabling a collaborative AI agent to consider its human partner's beliefs about its intentions, i.e., what the human partner thinks the AI agent is trying to accomplish, and to design its action plan accordingly to facilitate more effective human-AI collaboration. Specifically, we developed a model of human beliefs that captures how humans interpret and reason about their AI partner's intentions. Using this belief model, we created an AI agent that incorporates both human behavior and human beliefs when devising its strategy for interacting with humans. Through extensive real-world human-subject experiments, we demonstrate that our belief model more accurately captures human perceptions of AI intentions. Furthermore, we show that our AI agent, designed to account for human beliefs over its intentions, significantly enhances performance in human-AI collaboration.

==> 2_Related_Work_NeurIPS.tex <==
\section{Related Work}
%\subsection{Human in the loop reinforcement learning}
Our work contributes to the growing body of research on human-AI collaboration~\citep{carroll2019utility,jaderberg2019human,bansal2021most,wilder2021learning, myers2024learning}. For example, \citet{bansal2021most} demonstrate that optimizing AI in isolation may lead to suboptimal performance in human-AI collaboration, compared to training AI with consideration for human performance. \citet{wilder2021learning} show that training AI systems to complement humans by performing better in areas where humans struggle results in improved collaborative performance. \citet{carroll2019utility} illustrate that incorporating a human model, learned from human data, into the training of AI enhances performance when these AI systems collaborate with real humans.
Our work extends this line of research by not only accounting for human behavior when designing AI but also incorporating human beliefs about AI intentions.

While the approaches in the above works often assume knowledge or data of humans, there have also been zero-shot coordination techniques being proposed to train cooperative AI agents when human data are not available.  
For example, \citet{jaderberg2019human} use population-based reinforcement learning to improve the robustness of trained AI agents. 
\citet{strouse2021collaborating} develop a variety of self-play agents by varying random seeds of neural network initialization and various checkpoints, and train a best response model tailored to the agent population, discovering that humans prefer to partner with this model.
\citet{zhao2023maximum} utilize the advances of maximum entropy reinforcement learning to encourage the diversity of agent populations and show the learned AI models could adapt to real humans. 
This line of work aims to design collaborative AI that is robust to diverse human behavior. However, they do not explicitly account for human beliefs over AI intentions during human-AI collaboration. 
In this work, we have included these approaches as baselines and show that accounting for human beliefs lead to better performance in our setting.

From a technical perspective, our work focuses on understanding and modeling human decision-making. A significant body of literature has explored modeling human behavior. For example, inverse reinforcement learning (IRL)\citep{ng2000algorithms, abbeel2004apprenticeship, ramachandran2007bayesian} aims to infer reward functions in Markov decision processes (MDPs) by observing demonstrations of the optimal policy. When the demonstrator is human, these demonstrations may be noisy or exhibit behavioral biases. 
Several studies\citep{evans2016learning, shah2019feasibility, hughes2020inferring, zhi2020online} have addressed this by incorporating human behavioral biases into the inference process, aiming to infer both the rewards and biases simultaneously.
Imitation Learning~\citep{hussein2017imitation} also seeks to develop models that can mimic human behavior based on demonstrations.
Recently, there has been a growing amount of research that incorporates human models into computational and machine learning frameworks~\citep{KO-14, tang2019bandit, tang2021bayesian, egr2021, egr2021-2, yu2022environment, yu2023encoding, feng2024rationality, hong2024learning}.
% \ygh{Many existing behavioral cloning models are built upon data from human games only }


From the perspective of modeling human beliefs about others' intentions, this has been discussed in the literature on level-$k$ reasoning~\citep{stahl1994experimental,gill2016cognitive} in economics and in the theory of mind~\citep{premack1978does,chen2021visual, westby2023collective, li2023theory}. For instance, \citet{yu2006unified} found that real human behavior aligns closely with level-$1$ and level-$2$ reasoning models in cooperative games. \citet{albrecht2018autonomous} survey works on autonomous agents modeling the beliefs and intentions of other agents, distinguishing between methods for modeling stationary or changing agent behaviors.
These belief models include theory of mind, recursive reasoning models, plan recognition, partially observable Markov decision processes (POMDPs), and others. \citet{bara2021mindcraft} models human common ground in cooperative Minecraft tasks by leveraging theory of mind and develops AI models to infer human beliefs. \citet{baker2011bayesian} propose a Bayesian theory of mind to describe how humans model joint beliefs of state in a partially observable MDP, conducting human experiments in the works of~\citet{baker2009action, baker2017rational}. Similarly, \citet{wu2021too} apply a human modeling approach in the Overcooked experiment, breaking down the task of delivering a dish into several subtasks, such as picking up an ingredient or placing an ingredient into a pot, where the player infers others' intentions regarding these subtasks and selects their own accordingly before taking actions. 
Our work extends this line of research in two ways. 
First, our belief inference framework differs from previous theory of mind literature by modeling and incorporating human beliefs about AI intentions specifically, using a more realistic human model as the basis for inferring these intentions.
Second, and more importantly, beyond modeling human beliefs over others' intentions, our work focuses on the design of collaborative AI that account for human beliefs. 


% \ygh{add comparision with ToM, PBT/zeor-shot coordination,}

% Our approach relies on real human data. Another approach to design AI systems to cooperate with human is through zero-shot coordination. Prior work \cite{} show that reinforcement learning agents trained with diverse populations of partners could perform better than self-play agents in multi-player settings \cite{} or human-AI cooperation problems \cite{}. Our method show that when we have more realistic human behavior model, even a self-play agent could outperform the state-of-the-art zero-shot baselines. 

% level-$k$ reasoning\citep{gill2016cognitive} from game  describes how player make decisions based on their predictions of the likely actions of all other players.
% In previous human experiments, \citet{yu2006unified} find real human behavior is close to level-$1$ and level-$2$ reasoning model in cooperative game.
% \citet{albrecht2018autonomous} survey works on autonomous agents modeling belief and intention of other agents.
% They distinguish methods for modeling stationary or changing agent behaviors.
% The belief model includes theory of mind, recursive reasoning models, plan recognition, POMDP and others.
% \citet{baker2011bayesian} propose Bayesian theory of mind to describe human modeling joint belief of state in a partially observable MDP, and runs human experiments in \citep{baker2017rational, baker2009action}.
% A similar human modeling is adopted by \citet{wu2021too} and applied to the Overcooked experiment.
% Their idea is to split delivering a dish into several subtasks such as picking up an ingredient or putting ingredient into pot, and the player is inferring other's subtasks and select their own corresponding subtask before choosing actions.


%%% FIXME: Check later on what to include
% The belief model is also related to work in goal recognition and plan recognition, since the belief model is the future plan that other players will follow. 
% \citet{ramirez2010probabilistic} solve probabilistic goal recognition by updating posterior goal probability from a pre-defined planner.
% \citet{ramirez2011goal} infer intention of POMDP agent by goal recognition.
% Both approach use similar Bayesian ways to calculate posterior probabilities.

% Another approach is treating belief of other players as unknown state in decision-making, as POMDP.
% \citet{gmytrasiewicz2005framework} makes sequential inference of belief model by observed actions in such setting.
% \citet{rathnasabapathy2006exact} adapt this idea and combine with level-k reasoning model, iteratively find best response to solve a multi-agent POMDP problem.


% In \textbf{goal recognition}, \citet{keren2014goal} presents an exhaustive search method to minimize worst case distinctiveness (wcd) for optimal agents, and later \citet{keren2015goal} extends the method to non-optimal agent cases.
% \citet{min2016player} applies goal recognition methods to infer player goals in an open-world digital game with 153 middle school students.

% \citet{abbeel2004apprenticeship} proposes imitation learning techniques to infer human reward function from inverse reinforcement learning (IRL) and train agents to mimic human policy, and \citet{ho2016generative} advances such idea by generative adversarial networks to bypass the intermediate IRL step.
% Other work achieving human AI cooperation by learning human models (non-optimal) \citep{nikolaidis2013human} or designing specific reward function during training to aid cooperation \citep{dragan2013legibility}.
% Those models either increase generality or robustness of AI algorithms, or rely on a static human model (that is, human behavior is not changed no matter which teammate they are paired).

